Beyond Linearity and Time-Homogeneity: Relational Hyper Event Models with Time-Varying Non-Linear Effects

Recent technological advances have made it easier to collect large and complex networks of time-stamped relational events connecting two or more entities. Relational hyper-event models (RHEMs) aim to explain the dynamics of these events by modeling the event rate as a function of statistics based on past history and external information. However, despite the complexity of the data, most current RHEM approaches still rely on a linearity assumption to model this relationship. In this work, we address this limitation by introducing a more flexible model that allows the effects of statistics to vary non-linearly and over time. While time-varying and non-linear effects have been used in relational event modeling, we take this further by modeling joint time-varying and non-linear effects using tensor product smooths. We validate our methodology on both synthetic and empirical data. In particular, we use RHEMs to study how patterns of scientific collaboration and impact evolve over time. Our approach provides deeper insights into the dynamic factors driving relational hyper-events, allowing us to evaluate potential non-monotonic patterns that cannot be identified using linear models.

==> _FIGURES_/_SUPPLEMENTARY_EMPIRICAL.tex <==
\begin{figure}
    \centering
    \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_EMPIRICAL_/centered_plot_new_labels_author.sub.rep.1.pdf}
    \end{minipage}
    \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_EMPIRICAL_/centered_plot_new_labels_avg.author.citation.popularity.pdf}
    \end{minipage}
    \vspace{0.5em}
    \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_EMPIRICAL_/centered_plot_new_labels_collaborate.with.citing.author.pdf}
    \end{minipage}
    \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_EMPIRICAL_/centered_plot_new_labels_author.ref.paper.sub.rep.1.1.pdf}
    \end{minipage}
    \vspace{0.5em}
    \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_EMPIRICAL_/centered_plot_new_labels_diff.author.citation.popularity.pdf}
    \end{minipage}
    \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_EMPIRICAL_/centered_plot_new_labels_paper.outdegree.popularity.pdf}
    \end{minipage}
     \vspace{0.5em}
    \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_EMPIRICAL_/centered_plot_new_labels_reference.sub.rep.2.pdf}
    \end{minipage}
    \caption{\label{fig:empirical_supplementary} Estimated TVNLE that have not been included in the main text.}
\end{figure}

==> _FIGURES_/_SUPPLEMENTARY_FIGURE_RG_1.tex <==
\begin{figure}
    \centering
    \begin{minipage}{0.35\linewidth}
        \centering
        a) n = 5000 (Linear vs NLE Model)\\
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_1_/_FIG_SIM_LINEAR_NEWp20_n5000_m4_lin1.pdf}
    \end{minipage}
    \begin{minipage}{0.35\linewidth}
        \centering
        b) n = 10000 (Linear vs NLE Model) \\
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_1_/_FIG_SIM_LINEAR_NEWp20_n10000_m4_lin1.pdf}
    \end{minipage}
    
    \vspace{0.5em}
    
    \begin{minipage}{0.35\linewidth}
        \centering
        a) n = 5000 (Linear vs NLE Model) \\
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_1_/_FIG_SIM_LINEAR_NEWp20_n5000_m4_lin2.pdf}
    \end{minipage}
    \begin{minipage}{0.35\linewidth}
        \centering
        b) n = 10000 (Linear vs NLE Model) \\
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_1_/_FIG_SIM_LINEAR_NEWp20_n10000_m4_lin2.pdf}
    \end{minipage}
    
    \vspace{0.5em}
    
    \begin{minipage}{0.35\linewidth}
        \centering
        a) n = 5000 (Linear vs NLE Model) \\
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_1_/_FIG_SIM_LINEAR_NEWp20_n5000_m4_lin4.pdf}
    \end{minipage}
    \begin{minipage}{0.35\linewidth}
        \centering
        b) n = 10000 (Linear vs NLE Model) \\
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_1_/_FIG_SIM_LINEAR_NEWp20_n10000_m4_lin4.pdf}
    \end{minipage}
    \caption{\label{fig:simulation_study_linear_supplementary}\textbf{Linear models are recovered by penalized non-linear models.} Panels a) and b) display results based on synthetic data generated according to the model in Equation~(9), differing only in the number \(n\) of simulated events.
    Across experiment replications, estimates are aggregated using inverse variance weighting\index{inverse variance weighting}. For the linear model, this yields a consensus slope referred to as the \enquote{consensus linear effect} (blue dashed line). For non-linear models, predicted effects are interpolated across the covariate domain, and aggregated pointwise using inverse variance weights, resulting in the \enquote{consensus non-linear effect} (black dashed line). Since non-linear estimates are identifiable only up to an additive constant, the consensus curve is manually shifted for alignment. Confidence intervals, derived from the 5th and 95th percentiles of the empirical interpolated estimates at each covariate value, are also shifted accordingly. Both linear and non-linear estimated effects are compared to the ground truth (red solid line).}
\end{figure}

==> _FIGURES_/_SUPPLEMENTARY_FIGURE_RG_2.tex <==
\begin{figure}
    \centering
    
    \begin{minipage}{0.45\linewidth}
        \centering
        a) w = 4 (Linear vs TVE Model) \\
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_2_/_FIG_SIM_TV_p20_n5000_m4_TV1.pdf}
    \end{minipage}
    \begin{minipage}{0.45\linewidth}
        \centering
        b) w = 8 (Linear vs TVE Model) \\
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_2_/_FIG_SIM_TV_p20_n5000_m8_TV1.pdf}
    \end{minipage}
    
    \vspace{0.5em}
    
    \begin{minipage}{0.45\linewidth}
        \centering
        a) w = 4 (Linear vs TVE Model) \\
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_2_/_FIG_SIM_TV_p20_n5000_m4_TV2.pdf}
    \end{minipage}
    \begin{minipage}{0.45\linewidth}
        \centering
        b) w = 8 (Linear vs TVE Model) \\
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_2_/_FIG_SIM_TV_p20_n5000_m8_TV2.pdf}
    \end{minipage}
    \caption{\label{fig:simulation_study_tve_supplementary}\textbf{Linear models fail to capture non-linear effects.}  
    Panels a), b), display results based on synthetic data generated according to the model in (10), differing only in the maximum number \(w\) of participants allowed in a meeting. Estimates from multiple replications are combined using inverse variance weighting\index{inverse variance weighting}. For the linear model, we aggregate the estimated slopes to create a consensus line, called the \enquote{consensus linear effect} (blue dashed line). Unlike Figure~\ref{fig:simulation_study_linear_supplementary}, the x-axis here shows time. As a result, the consensus linear effect appears as a horizontal line, since it does not change over time. In contrast, the true effect (red solid line) changes over time. Linear models cannot capture this time-dependent pattern. For time-varying effects, we first interpolate predicted effects across time points. Then, we aggregate them pointwise, weighting each by the inverse of its variance. This produces a \enquote{consensus time-varying effect} (black dashed line) that captures the average time trend well. Notably, unlike in Figure~\ref{fig:simulation_study_linear_supplementary}, the sign of the effect here can be interpreted. Therefore, the consensus non-linear effect is not shifted.}
\end{figure}

==> _FIGURES_/_SUPPLEMENTARY_FIGURE_RG_3.tex <==
\begin{figure}
    \centering
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_3_/_FIG_SIM_TVNL_p20_n5000_m4_TV1.pdf}
    \end{minipage}
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{_FIGURES_/_SUPPLEMENTARY_/_RG_3_/_FIG_SIM_TVNL_p20_n5000_m4_TV2.pdf}
    \end{minipage}
    \caption{\label{fig:simulation_study_tvnle_supplementary}%
    \textbf{Time-varying effects for sub-repetition covariates}. This figure shows the estimated effects for the order 1 and 2 sub-repetition covariates within the model that includes TVNLE. These covariates are transformed using the log-square root function, as in the previous section. Their effect remains purely time-varying.}
\end{figure}

==> _SECTIONS_/closing_blinded.tex <==
\section{Acknowledgments}

This work was supported by the Swiss National Science Foundation [grant 192549]; and the Deutsche Forschungsgemeinschaft (DFG) [Project No. 555455503].

\section{Declaration of interest}

None.

\newpage
\bibliographystyle{plainnat}  
\bibliography{_REFERENCES_.bib}  

==> _SECTIONS_/title_blinded.tex <==
\title{Beyond Linearity and Time-Homogeneity: \\
Relational Hyper Event Models \\ with Time-Varying Non-Linear Effects}

\author{}

